Seeing isn't Believing: Practical Adversarial Attack Against Object Detectors

In this paper, we presented systematic solutions to build robust and practical AEs against real world object detectors. Particularly, for Hiding Attack (HA), we proposed the feature-interference reinforcement (FIR) method and the enhanced realistic constraints generation (ERG) to enhance robustness, and for Appearing Attack (AA), we proposed the nested-AE, which combines two AEs together to attack object detectors in both long and short distance. We also designed diverse styles of AEs to make AA more surreptitious. Evaluation results show that our AEs can attack the state-of-the-art real-time object detectors (i.e., YOLO V3 and faster-RCNN) at the success rate up to 92.4% with varying distance from 1m to 25m and angles from -60{\deg} to 60{\deg}. Our AEs are also demonstrated to be highly transferable, capable of attacking another three state-of-the-art black-box models with high success rate.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> Overview.tex <==
%-------------------------------------------------------------------------------
\section{Overview}
\label{sec:overview}

In this section, we present the motivation to our research, and then overview the approach.  

\subsection{Motivation}

Initially inspired by an accident of self-driving car (Tesla Model S) which failed to distinguish a large white 18-wheel truck with the bright sky in May 2016~\cite{TeslaAccident}, we thought whether there exists such an attack that can fool the object detector in the self-driving car to make it fail to recognize some important targets such as stop signs (referred to as \textit{hiding attack}, or \textit{HA} in short) or to recognize an non-existence object (referred to as \textit{appearing attack} or \textit{AA} in short). As we know, the key algorithm utilized in object detectors recently is deep learning, which is known to be vulnerable to adversarial samples. We want to know whether such samples can attack object detectors in reality. 

\Shengzhi{The paragraph below does not read like motivation. Probably examples in Threat Model?}

However, it is quite challenging to achieve practical adversarial attacks on real object detectors. Figure~\ref{Mimic diagram of appearance attack.} shows an example. The left part of the image shows an scenario of \textit{hiding attack}, an autonomous car is running on a straight road with a stop sign on its side. And there is a crossroad ahead. Assuming the stop sign is our attack target. We will add perturbations on it to make it disappear from the view of the car. Note that the car is moving along the road while perturbations are still. So the stop sign captured by the object detector in the car looks different (with different sizes and angles). For example, in the figure, we show the four views by the car in four different positions (i.e., A, B, C, D). Similarly, the appearing attack is shown on right part of Figure~\ref{Mimic diagram of appearance attack.}. We want to let the car stop by creating a stop sign using an adversarial sample. If this happens, the car will stop or slow down suddenly in the road, potentially causing serious accidents. Still, the adversarial samples look different from the four different positions (i.e., A, B, C, D). So our practical adversarial examples against the object detector are facing two main challenges: \yue{(Q1) Is it possible to build a practical AEs which could be robust enough against different distances, angles and illuminations on continuous video frames? (Q2) Is it feasible to generate the AEs in an unnoticeable way?} \yuee{(Q3) If the answer for Q1 is Yes, could this kind of AEs keep high success rate against the black-box detectors?}

\Shengzhi{Can we reuse the challenges summarized in Introduction? Some of the questions are redundant to the challenges.}

\subsection{Insights}
\Shengzhi{Redundant to Introduction? How about overviewing the approach here based on the flow chart (the picture uploaded by Kai)? So we focus on the workflow, rather than how each problem is solved here.}

Regarding Q1, instead of using the small perturbations as the AEs to attack the object detectors in digital world, we choose larger adversarial patterns to attack detectors in physical world. This is mainly because small perturbations are very hard to be caught by cameras which are the front-end of object detectors in physical world, especially when the distances and angles vary. Hence we choose to increase the size of perturbations (referred to as \textit{sticker} in this paper), which should be robust against the relatively low perception capability of cameras. 


Furthermore, we introduce the image transformation methods to simulate the varying factors including distances, angles, backgrounds, printer chromatic aberrations and illumination changes. As we know, captured from different angles, the images will face different illumination conditions and color aberration. As shown in Figure~\ref{Implemantation.}, the transformation includes perspective transformation, rescaling transformation, gray-scale transformation and random background. We also include random noise for increasing the robustness. For AA, besides the image transformations, we also propose \textit{nested AEs} to improve the robustness of AEs. Nested AEs is a combination of two adversarial pattern as shown in Figure~\ref{effectiveness against attack.}. The inner pattern can attack the object detector from short distance while the whole patch works for long distance. From our evaluation, we find that this approach extends the distance from 6 to 25 meters. After the transformations, the perturbations can be calculated by iterative fast gradient sign method (I-FGSM). Different from HA, AA does not need to train with the picture of a stop sign. The generated perturbations can be added to different regions in a single patch according to the re-scaling size. 

\yue{Regarding Q2, we introduced the style-based AEs generating method to disguise the our AEs as the normal stickers like the small ads stickers or graffiti. We generate small ads style AEs by introducing English letters and gray colors and generate graffiti style stickers through pattern control, color control and shape control methods. Pattern control aims to generate patches with specified interesting target patterns like the clock, person or animals, and the shape control makes patches to be various in shape and the color control generates patches with specified color hue such as the red hue.}

\yuee{Regarding Q3, we proposed the batch-variation momentum method to improve the transferability of Mal-stickers. .}


%-------------------------------------------------------------------------------
